Progressive Fourier Neural Representation for Sequential Video Compilation

Neural Implicit Representation (NIR) has recently gained significant attention due to its remarkable ability to encode complex and high-dimensional data into representation space and easily reconstruct it through a trainable mapping function. However, NIR methods assume a one-to-one mapping between the target data and representation models regardless of data relevancy or similarity. This results in poor generalization over multiple complex data and limits their efficiency and scalability. Motivated by continual learning, this work investigates how to accumulate and transfer neural implicit representations for multiple complex video data over sequential encoding sessions. To overcome the limitation of NIR, we propose a novel method, Progressive Fourier Neural Representation (PFNR), that aims to find an adaptive and compact sub-module in Fourier space to encode videos in each training session. This sparsified neural encoding allows the neural network to hold free weights, enabling an improved adaptation for future videos. In addition, when learning a representation for a new video, PFNR transfers the representation of previous videos with frozen weights. This design allows the model to continuously accumulate high-quality neural representations for multiple videos while ensuring lossless decoding that perfectly preserves the learned representations for previous videos. We validate our PFNR method on the UVG8/17 and DAVIS50 video sequence benchmarks and achieve impressive performance gains over strong continual learning baselines. The PFNR code is available at https://github.com/ihaeyong/PFNR.git.

==> materials/plot_psnr_bpp.tex <==
\begin{figure}[h]
    \centering
    \small
    \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    \includegraphics[width=0.5\columnwidth]{images/psnr/UVG17B_psnr_bit_UVG17B.pdf} & 
    \includegraphics[width=0.5\columnwidth]{images/psnr/UVG17B_psnr_bpp_UVG17B.pdf} \\
    \small (a) Quantization and Compression of PNR, \textcolor{red}{reinit} & \small (b) PSNR v.s. BPP
    \end{tabular}
    }
    \caption{\small PSNR v.s. Bits-per-pixel (BPP) on the UVG17 datasets }
    \label{fig:psnr_bit_bpp}
    \vspace{-0.12in}
\end{figure}

==> materials/plot_reinit_capacity.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/psnr/UVG17B_psnr_UVG17B.pdf} & 
    %\includegraphics[width=0.5\columnwidth]{images/capacity/UVG17B_capacity_UVG17B.pdf} \\
    \includegraphics[width=0.5\columnwidth]{images/capacity/UVG17B_reinit_capacity_UVG17B.pdf} \\
    \small (a) PSNR, ExNIR with $c = 30.0\%$ & \small (b) ExNIR'capacity with $c = 30.0\%$, \textcolor{red}{reinit} \\
    \end{tabular}
    }
    \caption{ExNIR's Comparisons with others and layer-wise Capacities on the UVG 17 dataset. Note that green represents a reused subnetwork at the current session (s) obtained at the past (s-1) video sessions in (b).}
    \label{fig:psnr_comp}
    \vspace{-0.12in}
\end{figure}

==> materials/plot_wsn_capacity.tex <==
\begin{figure}[ht]
    \centering
    \small
    %\vspace{-0.1in}
    \setlength{\tabcolsep}{0pt}{%
    \begin{tabular}{cc}
    % we prepare the figure 
    \includegraphics[width=0.5\columnwidth]{images/psnr/WSN_psnr_UVG17B.pdf} &
    %\includegraphics[width=0.5\columnwidth]{images/psnr/PFNR_psnr_UVG17B.pdf} &
    %\includegraphics[width=0.5\columnwidth]{images/capacity/UVG17B_capacity_UVG17B.pdf} \\
    \includegraphics[width=0.5\columnwidth]{images/capacity/UVG17B_reinit_capacity_UVG17B.pdf} \\
    \small (a) PSNR, WSN with $c = 30.0\%$ & \small (b) WSN'capacity with $c = 30.0\%$ \\
    \end{tabular}
    }
    \caption{\small PNR's Comparison of PSNR with others and layer-wise accumulated Capacities on the UVG17 dataset. Note that \textcolor{green}{green} represents a reused subnetwork at the current session (s) obtained at the past (s-1) video sessions in (b): \textcolor{red}{reinit} (solid line) v.s \textcolor{cyan}{non-reinit} (dashed line) \textcolor{blue}{of fully-connected (fc1, $\circ$), layers (1, $\triangledown$) and (4, $\square$).}}
    \label{fig:psnr_cap}
    %\vspace{-0.12in}
\end{figure}
